Information Types in Product Reviews

Information in text is communicated in a way that supports a goal for its reader. Product reviews, for example, contain opinions, tips, product descriptions, and many other types of information that provide both direct insights, as well as unexpected signals for downstream applications. We devise a typology of 24 communicative goals in sentences from the product review domain, and employ a zero-shot multi-label classifier that facilitates large-scale analyses of review data. In our experiments, we find that the combination of classes in the typology forecasts helpfulness and sentiment of reviews, while supplying explanations for these decisions. In addition, our typology enables analysis of review intent, effectiveness and rhetorical structure. Characterizing the types of information in reviews unlocks many opportunities for more effective consumption of this genre.

==> Figures/table_downstream_experiments_description.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
                 & & \multirow{2}{*}{\makecell{Helpful\\Reviews}} & \multirow{2}{*}{\makecell{Helpful\\Sentences}} & \multirow{2}{*}{\makecell{Sentiment\\Analysis}} \\
        %\diagbox{Type Set}{Task} & & & \\
        \multicolumn{2}{l}{Method} & & \\
        \midrule
        \multirow{6}{*}{\rotatebox[origin=c]{90}{{\small\taxtype{} Set with SVM}}} & subjective      & 69.6 & 82.1 & 83.7 \\
        & ~~~(\textit{opinion} only)    & 48.7 & 72.7 & 80.2 \\
        & ~~~(\textit{op. w/rsn.} only) & 67.4 & 80.9 & 80.2 \\
        & objective       & 67.3 & 83.3 & 80.2 \\
        & stylistic       & 63.1 & 63.7 & 84.0 \\
        \cmidrule{2-5}
        & \textbf{All \taxtypes{}} & 72.6 & 88.3 & 88.1 \\
        \midrule
        \multicolumn{2}{l}{Coarse-grained types w/SVM} & 67.7 & 85.9 & 80.4 \\
        \multicolumn{2}{l}{Random (50-50)}             & 50.0 & 50.0 & 50.0 \\
        \multicolumn{2}{l}{Random (proportion known)}  & 50.0 & 51.0 & 68.3 \\
        \bottomrule
    \end{tabular}}
    \caption{Accuracy scores (\%) on the classification tasks using an SVM with different subsets of \taxtypes{} (\autoref{tab_taxonomy_groups}) from the typology (top). The combination of all \taxtypes{} best predicts helpfulness and sentiment. The bottom part shows prediction results using the coarse-grained types from \autoref{tab_taxonomy_groups} as features to an SVM, and the results of random predictors. Full results are in \autoref{tab_classification_results_full} in the appendix.}
    \label{tab_classification_results}
\end{table}

==> Figures/table_predictor_eval_all_old.tex <==
\begin{table*}[th]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrc}
        \toprule
        & \multicolumn{3}{c}{Recall@Precision} & & \multirow{2}{*}{\makecell{Train/Test \\ Size}}\\
        \textit{Tip} Classifier & 75 & 80 & 85 & $F_1$ \\
        \midrule
        \citeauthor{hirsch2021producttips} Best BL & 43.4 & 29.0 & 16.8 & - & 4894/1224 \\
        \citeauthor{hirsch2021producttips} BERT    & 70.5 & 58.1 & 36.1 & - & 4894/1224 \\
        Ours                        & 42.6 & 32.6 & 32.2 & 61.4 & 6156/1540 \\
        Ours (no \textit{warning}s) & 63.7 & 49.8 & 40.9 & 71.0 & \underline{4140}/1036 \\
        Ours (no \textit{warning}s) & 63.7 & 49.7 & 40.3 & 70.0 & \underline{100}/1036 \\
        \bottomrule
    \end{tabular}
    \quad
    \begin{tabular}{ccc}
        \toprule
        Our Classifier & & \multirow{2}{*}{\makecell{Train/Test \\ Size}}\\
        on \taxtype{}  & $F_1$ \\
        \midrule
        \multirow{2}{*}{\makecell{\textit{Opinion}}}   & 87.6 & \underline{3105}/1386 \\
           & 85.8    & \underline{100}/1386 \\
        \midrule
        \multirow{2}{*}{\makecell{\textit{Opinion} \\ \textit{w/ Reason}}}   & 62.8 & \underline{1221}/501 \\
           & 62.8    & \underline{100}/501 \\
        \midrule
        \multirow{1}{*}{\makecell{All}}   & 56.7 & 300/240 \\
        \bottomrule
    \end{tabular}}
    \caption{Results on \taxtype{} classification benchmarks, and our direct evaluation test set -- \textit{Tip} \taxtype{} on the left, and opinion \taxtypes{} and direct evaluation on the right. No direct $F_{1}$ results have been reported on the \taxtype{}-specific source datasets. The underlines emphasize the difference in the size of the train set, which, in our case, is only used for tuning the \taxtype{} threshold. For the direct evaluation, the types were tuned on our development set.}% \uvp{Reshape to make sense with the opinion results as well (maybe `no warnings' and `limited data' as separate columns under a \emph{tips} meta-column)}}
    \label{tab_predictor_all_benchmark}
%    \caption{a}
%    \label{}
\end{table*}


        %\citeauthor{hirsch2021producttips} Best BL & 43.4 & 29.0 & 16.8 & 15.3 & - & 4894/1224 \\
        %\citeauthor{hirsch2021producttips} BERT & 70.5 & 58.1 & 36.1 & 19.3 & - & 4894/1224 \\
        %Ours          & 42.6 & 32.6 & 32.2 & -    & 61.4 & 6156/1540 \\
        %Ours (no \textit{warning}s)& 63.7 & 49.8 & 40.9 & -    & 71.0 & \underline{4140}/1036 \\
        %Ours (no \textit{warning}s)& 63.7 & 49.7 & 40.3 & -    & 70.0 & \underline{100}/1036 \\

==> Figures/table_tips_results_vs_baseline.tex <==
\begin{table}[th]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        & \multicolumn{3}{c}{Recall@Precision} \\
        \textit{Tip} Classifier & 75 & 80 & 85 \\
        \midrule
        \citeauthor{hirsch2021producttips} Best Baseline & 43.4 & 29.0 & 16.8 \\
        \citeauthor{hirsch2021producttips} Best (BERT)   & 70.5 & 58.1 & 36.1 \\
        Ours (no \textit{warning}s)                         & 63.7 & 49.7 & 40.3 \\
        %Ours                                       & 42.6 & 32.6 & 32.2 \\
        %Ours* (no \textit{warning}s)               & 63.7 & 49.7 & 40.3 \\
        \bottomrule
    \end{tabular}}
    \caption{Results on the \textit{Tip} classification benchmark of \citet{hirsch2021producttips}. We only use 100 train instances for tuning the \textit{Tip} \taxtype{} threshold. We removed the \textit{warning} sub-type from the data to better represent our notion of a \textit{tip}.}
    %\caption{Results on the \textit{Tip} classification benchmark of \citet{hirsch2021producttips}. The * signifies we only use 100 train instances for tuning the \textit{Tip} \taxtype{} threshold. Using the full train set improves results insignificantly.}
    \label{tab_tips_results_vs_baseline}
\end{table}

==> related_work.tex <==
%scientific articles contain 
%news/media coverage -> stance, framing
%debate -> argument claim and premise
%scientific -> background, proof
%reviews -> sentiment, tips
%blog/forums -> toxicity
%user requests -> intent detection
%email -> spam or intent


Categorizing texts into classes or taxonomies has been researched extensively across domains and on different lengths of texts.

Sentence-level taxonomies:
\citep{core1997dialog_annotation, jurafsky1997discourse_structure} define annotation scheme for communicative acts in dialog, part of which addresses the form and content. \citep{khoo2006email_classification} on intents and communicative forms in emails.

\citep{yu2012product_title_categories} product title classification to the product category.

\citep{li2002question_classification} question multi-label classification into a taxonomy of answer types as adopted from TREC (6 classes).

\citep[SST][]{socher2013finegrained_sentiment} fine-grained (5-class) sentiment analysis of movie review phrases.

\citep{pang2004subjective_reviews} subjective/objective sentence or phrases in movie reviews.

\citep{guo2019sentence_classification_dl} use augmented CNNs and LSTMs to solve sentence classification on several benchmarks and domains.

\citep{chai2020rl_classification} yse RL across benchmarks and domains for single-label and mlti-label.

\citep{go2009sentiment_distant} use distant supervision for sentiment analysis on micro-blog posts.

\citep{Brack2022classification_transfer} use a hierarchical transformer-based \citep{beltagy2019scibert} model and show how to effectively train the model so that it transfers across domain for sentence classification.

Product insights:
\citep{hirsch2021producttips} product tips from reviews. Also talk about different kinds of sentences (short, enthusiactic, listing-specific, personal) that are usually not tips, and use lexical match heuristically to find these.


\citep{yin2019zeroshot_classification} study zero-shot text classification and propose an NLI-based framework for it.

\citep{zhang2021zeroshot_classification} zero-shot event and argument classification using SRL tools and a pre-trained LM.

\citep{Tesfagergish2022zeroshot_classification} zero-shot emotion classification using pre-trained language models that were trained on different nli tasks.

\citep{wiebe2005opinionAnnotation} annotation of opinions, emotions, sentiments, speculations, evaluations and other private states in language, in the news domain.

\citep{chen2022argumentMiningForHelpfulness} annotate arguments in reviews at the level of opinions/facts and evidence, and show its relation to helpfullness of a review.

\citep{liu2017argsForHelpfullness} inject argument features to predict a review's helpfulness.
